First Results on UAV-aided User Localization Using ToA and OpenAirInterface in 5G NR

This paper considers the challenge of localizing ground users with the help of a radio-equipped unmanned aerial vehicle (UAV) that collects measurements from users. We utilize time-of-arrival (ToA) measurements estimated from the radio signals received from users collected by a UAV at different locations. Since the UAV's location might not be perfectly known, the problem becomes about simultaneously localizing the users and tracking the UAV's position. To solve this problem, we employed a least-squares simultaneous localization and mapping (SLAM) framework to fuse ToA data and the estimate of UAV location available from global positioning system (GPS). We verified the performance of the developed algorithm through real-world experimentation.

==> sections/TRJ_Optimization.tex <==
\section{UAV Trajectory Optimization}\label{sec:TrajectoryDesign}

Contrary to static anchors in wireless node localization systems, we can optimize the trajectory of the UAV (as a mobile anchor) to improve localization performance. Specifically, UAV path planning problems that constitute a good trajectory to collect the most informative measurements, among all feasible paths, satisfying a duration or energy budget constraint can be formulated. In machine learning and robotics, such an optimization framework is often referred to as active learning or optimal design of experiments \cite{taylor2021active}. The relevance of this problem to our localization scenario can be understood as follows: The measurements collected links that are far from the BS usually result in a degradation of the localization accuracy due to the lower signal-to-noise ratio (SNR) and higher probability of the link obstruction by the blocking objects in the environment (i.e. buildings). On the other hand, devising a trajectory for the UAV to maintain high SNR links to all users at all times is not a viable solution since there may not exist a continuous trajectory that fulfills this constraint and because of the limited mission time. Therefore, optimizing the UAV trajectory to strike a balance between collecting informative measurements from the users and the mission time is crucial.

To do so, in this section, we employ the the notion of Fisher information matrix (FIM) \cite{amari2007methods} to find a maximally informative UAV trajectory. This metric helps in measuring the amount of information that observed measurements carries about an unknown user locations and channel parameters.
Our goal is to exploit structural properties of the FIM, so as to design an optimal policy for the UAV to collect the best possible measurements from users. In the following, we briefly explain the FIM and its properties and then optimize the UAV's trajectory.

\subsection{Fisher Information Matrix}
For a set of ToA measurements collected by the UAV from users, the FIM of the measurements with respect to the users locations is given by
 \begin{equation}
     {\bf{F}} = \Exp\left[ \frac{\partial\mathcal{L}_{\text{UAV-UE}} }{\partial {\bf{u}}} {\frac{\partial\mathcal{L}_{\text{UAV-UE}}^{\tau}}{\partial {\bf{u}}}}^\Tr \right],
 \end{equation}
where ${\bf{u}}=[{\bf{u}}_1^{T},\cdots,{\bf{u}}_K^{T}]^{\Tr}$ is a vector stacking all the users locations, and $\mathcal{L}_{\text{UAV-UE}}$ is the log-likelihood of ToA measurements collected by the UAV from users defined as
 \begin{equation}
 \begin{aligned}
     \mathcal{L}_{\text{UAV-UE}} \triangleq &  \sum_{k=1}^{K}\sum_{n=1}^{N} \frac{1}{\sigma_{\tau}^2}  \left | \Hat{\tau}_{0, k}[n] - \frac{\|{\bf{x}}[n] - {\bf{u}}_k \|}{C}\right|^2.
      \end{aligned}
 \end{equation}
 The FIM for all measurements collected up to time step $N$ is then given by 
 \begin{equation}
 \begin{aligned}
          {\bf{F}}_{N} =& \sum_{n=1}^{N}\sum_{k=1}^K {\bf{H}}_{k}[n]\\
          =& \,{\bf{F}}_{N-1} + \sum_{k=1}^K {\bf{H}}_{k}[N], \label{eq:FIM_equation}
 \end{aligned}
 \end{equation}
 where ${\bf{H}}_{k,s}[n]$ is derived akin to \eqref{eq:graph_slam_hessian}. Note that, \eqref{eq:FIM_equation} implies that the FIM is cumulative over time.
 \subsection{Cramér-Rao Bound Analysis}
According to  the Cramér-Rao bound (CRB) \cite{van2007parameter}, the mean square error (MSE) of the estimated parameters ${\bf{u}}$ given the measurements for an unbiased estimator is lower bounded by 
   \begin{equation}
 \begin{aligned}
          \text{MSE}({\bf{u}})\ge\trace{({\bf{F}}_{N}^{-1})}, \label{eq:MSE_CRB_LB}
 \end{aligned}
 \end{equation}
\noindent where $\trace{({\bf{F}}_{N}^{-1})}$ is the trace of ${\bf{F}}_{N}^{-1}$. Using the matrix inversion lemma, it can be shown that ${\bf{F}}_{N,s}^{-1}$ follows a recursive relation as follows
 \begin{equation} \label{eq:FIM_recursion}
     {\bf{F}}_{N}^{-1} = {\bf{F}}_{1}^{-1} - \sum_{n=2}^{N}{\bf{R}}[n],
 \end{equation}
 where ${\bf{R}}[n]$ is defined as the amount of improvement in the estimate within time slot $n$ which is given by
 \begin{equation}
     {\bf{R}}[n] = {\bf{F}}_{n-1}^{-1}\left(\sum_{k=1}^K{\bf{H}}_{k}[n]^{-1}+{\bf{F}}_{n-1}^{-1}\right)^{-1}{\bf{F}}_{n-1}^{-1}.
 \end{equation}
 This recursion will be used later to optimize the UAV trajectory.
\subsection{Trajectory Optimization}
We aim to find a trajectory for the UAV starting from ${\bf{x}}_{\text{I}}$ and ending at the terminal point ${\bf{x}}_{\text{F}}$ under a constraint flight mission time to minimize the estimation error of parameters ${\bf{u}}$. Such optimization problem can be formulated as
\begin{subequations}\label{eq:TRJ_OPT_Origin}
 \begin{align}
  \begin{split}
          \min_{\{{\bf{x}}[n]\}_{n=1}^N} &\quad \text{MSE}({\bf{u}}) \label{eq:TRJ_OPT_Origin_O.F.}
 \end{split}\\
   \begin{split}
          \text{s.t.}&\quad
           {\bf{x}}[1] = {\bf{x}}_{\text{I}},\, {\bf{x}}[N] = {\bf{x}}_{\text{F}}, \label{eq:TRJ_OPT_Origin_x_t}
 \end{split}\\
 \begin{split} \label{eq:TRJ_OPT_max_speed}
           &\quad \| {\bf{x}}[n] - {\bf{x}}[n-1] \| \le D_{\text{max}}, \, n \in [2, N],
 \end{split}
 \end{align}
\end{subequations}
where $D_{\text{max}}$ is the maximum distance that the UAV can travel within each time step. The optimization problem \eqref{eq:TRJ_OPT_Origin} is challenging since a closed form solution for $\text{MSE}({\bf{u}})$ is not available. Therefore, we alternatively find a trajectory to minimize the CRB. Note that even though CRB in \eqref{eq:MSE_CRB_LB} only applies for unbiased estimators, in this case it nonetheless provides a good metric for finding favorable measurements in our trajectory optimization.
Using the CRB in \eqref{eq:MSE_CRB_LB}, we can approximate \eqref{eq:TRJ_OPT_Origin}
as
   \begin{subequations}\label{eq:TRJ_OPT_LB_Rec}
 \begin{align}
  \begin{split}
          \min_{\{{\bf{v}}[n]\}_{n=1}^N} &\quad \trace{({\bf{F}}_{N}^{-1})} 
 \end{split}\\
    \begin{split}
          \text{s.t.}&\quad \eqref{eq:TRJ_OPT_Origin_x_t}, \eqref{eq:TRJ_OPT_max_speed}.
 \end{split}
  \end{align}
  \end{subequations}
Even after this approximation of the original problem, \eqref{eq:TRJ_OPT_LB_Rec} is still not easy to solve. The non-linearity nature of user locations makes 
${\bf{F}}_{N}^{-1}$ a function of the unknown parameters ${\bf{u}}_k$ (that need to be estimated), hence
can not be computed exactly. To avoid this, we take a sequential approach where at time step $n$, we use an estimate of ${\bf{F}}_{N}^{-1}$, denoted by $\hat{\bf{F}}_{N|n}^{-1}$, as the objective to minimize. This estimate is obtained from using 
$\hat{{\bf{u}}}_{k, n}$, which represents an estimate of ${\bf{u}}_k$
obtained from measurements collected up to the time slot $n$.
Essentially, \eqref{eq:TRJ_OPT_LB_Rec} turns into an online learning and path planning problem. At each time step during the mission, new measurements are obtained, and then the estimates for unknown parameters are updated. Based on these updates, a new trajectory is generated from that point. In the following section, we will provide details on an online and low-complexity greedy algorithm that can be used to find a sub-optimal trajectory.

  \subsection{Greedy Trajectory Design} \label{sec:greedy_trj_design}
In this section, we present a greedy approach that involves designing the trajectory locally and piece by piece. At each time step, the UAV aims to identify the best location for the next step in order to gather measurements that could potentially lead to the maximum improvement in the estimation error. The objective function in the greedy algorithm at time step $n$ is defined as:
 \begin{equation} \small
      L({\bf{x}}[n]) = \left\{\begin{array}{rcl}
        \trace{(\hat{\bf{R}}_{n|n-1})}, & \|{\bf{x}}[n]-{\bf{x}}_{\text{F}}\|\le \tau\\
        -\infty ,& \text{otherwise}
      \end{array}\right. ,\label{eq:Greedy_Cost}
  \end{equation}
where $\hat{\bf{R}}_{n|n-1}$ is the estimation of ${\bf{R}}[n]$ given $\hat{{\bf{u}}}$, and $\tau=D_{\text{max}} (N-n)$.
Note that the relation between $\hat{\bf{R}}_{n|n-1}$ and $\hat{\bf{F}}_{N|n-1}$ can be inferred from \eqref{eq:FIM_recursion}.  
The definition in \eqref{eq:Greedy_Cost} forces the UAV to reach the terminal point ${\bf{x}}_{\text{F}}$ within the total flying time constraint.

Finally, the next optimal UAV position at any time step $n\in [1,N-1]$ can be obtained by solving
\begin{equation} \label{eq:Re_Greedy_TRJ_UAV_model}
\begin{aligned}
\max_{{\bf{x}}[n]}
&\quad L({\bf{x}}[n+1])\\
\text{s.t.} 
& \quad {\bf{x}}[1] = {\bf{x}}_{\text{I}},\\
& \quad \| {\bf{x}}[n+1] - {\bf{x}}[n] \| \le D_{\text{max}}.
\end{aligned} 
\end{equation}
\noindent To solve problem \eqref{eq:Re_Greedy_TRJ_UAV_model}, we initialize $n=1$ and the UAV starts flying from base point ${\bf{x}}[1] = {\bf{x}}_{\text{I}}$. To find the best UAV position in the next time step $({\bf{x}}[n+1], n\in [1,N-1])$, we discretize the search space around the current UAV location and we calculate \eqref{eq:Greedy_Cost} for all adjacent points. Then the neighbor point with the maximum value is chosen as the UAV next location. If the value of all the adjacent point are calculated as infinity, then the UAV moves towards the terminal location ${\bf{x}}_{\text{F}}$ by $\frac{\|{\bf{x}}[n]-{\bf{x}}_{\text{F}}\|}{N-n}$ meters, where $n$ is the current time step.
